Robust and Sample Optimal Algorithms for PSD Low-Rank Approximation

Recently, Musco and Woodruff (FOCS, 2017) showed that given an $n \times n$ positive semidefinite (PSD) matrix $A$, it is possible to compute a $(1+\epsilon)$-approximate relative-error low-rank approximation to $A$ by querying $O(nk/\epsilon^{2.5})$ entries of $A$ in time $O(nk/\epsilon^{2.5} +n k^{\omega-1}/\epsilon^{2(\omega-1)})$. They also showed that any relative-error low-rank approximation algorithm must query $\Omega(nk/\epsilon)$ entries of $A$, this gap has since remained open. Our main result is to resolve this question by obtaining an optimal algorithm that queries $O(nk/\epsilon)$ entries of $A$ and outputs a relative-error low-rank approximation in $O(n(k/\epsilon)^{\omega-1})$ time. Note, our running time improves that of Musco and Woodruff, and matches the information-theoretic lower bound if the matrix-multiplication exponent $\omega$ is $2$. We then extend our techniques to negative-type distance matrices. Bakshi and Woodruff (NeurIPS, 2018) showed a bi-criteria, relative-error low-rank approximation which queries $O(nk/\epsilon^{2.5})$ entries and outputs a rank-$(k+4)$ matrix. We show that the bi-criteria guarantee is not necessary and obtain an $O(nk/\epsilon)$ query algorithm, which is optimal. Our algorithm applies to all distance matrices that arise from metrics satisfying negative-type inequalities, including $\ell_1, \ell_2,$ spherical metrics and hypermetrics. Next, we introduce a new robust low-rank approximation model which captures PSD matrices that have been corrupted with noise. While a sample complexity lower bound precludes sublinear algorithms for arbitrary PSD matrices, we provide the first sublinear time and query algorithms when the corruption on the diagonal entries is bounded. As a special case, we show sample-optimal sublinear time algorithms for low-rank approximation of correlation matrices corrupted by noise.

==> adaptive_sampling.tex <==
\section{Adaptive Sampling}
In this section, we describe an algorithm that adaptively samples entries in $\AA$ to output a set of $\widetilde{O}\hspace{-0.1cm}\left(\frac{k}{\epsilon}\right)$ rows of $\AA$ such that running \cite{fkv04} on this subset of rows results in a subspace that contains a good additive error low-rank approximation to $\AA$. The algorithm is as follows :

\begin{Frame}[\textbf{Algorithm \ref{alg:adaptive}} : Adaptive Sampling for PSD Low-Rank Approximation]
\label{alg:adaptive}
\textbf{Input}: A PSD Matrix $\AA_{n \times n}$, integer $k$
\begin{enumerate}
    \item Sample $\Theta(n)$ entries uniformly at random from $\AA$ and rescale such that $\tilde{v}^2 = \Theta(\|\AA\|^2_F)$. 
    \item For $t \in [\log(n)]$, let $\BB^{t}$ be a $\frac{n}{2^t} \times n$ matrix such that  $\BB^{t}_{i,*} = \AA_{i',*}$ with probability $\frac{1}{2^t}$ for all $i' \in [n]$.
    \begin{enumerate}
        \item Let $r_t = \frac{2^t k \log(n)}{\epsilon}$. For $i \in \left[\frac{n}{2^t} \right]$,  sample $r_t$ entries from $\BB^t_{i,*}$ uniformly at random. Let $\CC^t_{i}=\{X_{i,1} \ldots X_{i,r_t}\}$ be the resulting set such that $X_{i, j}= (\BB^t_{i,j'})^2$ with probability $\frac{1}{n}$, for all $j' \in [n]$. Let $\CC^t$ be the resulting random matrix.  
        \item Partition  $\CC^t$ into level sets, i.e.  $\CC^t = \bigcup_{\ell \in [\log(n)]} \DD^{t,\ell} $ such that all entries of $\DD^{t,\ell}$ have absolute value in the range $\left( \frac{1}{2^{\ell+1}}, \frac{1}{2^\ell}\right]$.  
        \item  For all $\ell \in [\log(n)]$, for all $i \in [\frac{n}{2^t}]$, let $\S_{t,\ell} = \phi$. If $\DD^{t,\ell}_{i,*}$ contains $c$ entries, for a fixed constant $c$, $\S_{t,\ell} :=\S_{t,\ell} \bigcup \{ i \} $. Let $\R_{t,\ell}$ be a uniform subset of $\S_{t,\ell}$ such that $|\R_{t,\ell}| \leq \frac{k\log(n)}{\epsilon}$.  Read all rows in $\AA$ corresponding to the indices in $\R_{t,\ell}$.  
        \item Let $\tau_t \geq \frac{\tilde{v}}{2^t}$. Let $\I_t \subset [n]$ be the set of indices corresponding to rows of  $\AA$ read in the above step. For $i' \in [n]$, if $\|\AA_{i',*}\|^2_2 \geq \tau_t$, $\I_t := \I_t \bigcup \{i'\}$.
    \end{enumerate}
    \item Let $\I = \bigcup_t \I_t $. Run Frieze-Kannan-Vempala with the rows of $\AA$ indexed by $\I$ as input.
    \item Let $\MM \in \mathbb{R}^{n \times k}$ and $\NN \in \mathbb{R}^{k \times n}$ be the resulting matrices output by Frieze-Kannan-Vempala. 
\end{enumerate}
\textbf{Output: $\MM \cdot \NN^T$}  
\end{Frame}
We begin by bounding the total number of entries read by Algorithm \ref{alg:adaptive}. The sample complexity of the non-adaptive step (2a) of our algorithm is easy to bound. For the adaptive part, it may be the case that most rows of $\AA$ pass the test we construct. Therefore, we have to explicitly limit the number of rows we read at a given level of subsampling. We show that for each level set, $\DD^{t,\ell}$, we consider we read at most $\frac{k\log(n)}{\epsilon}$ rows of $\AA$. Since there are at most $\log^2(n)$ such level sets, we restrict the overall sample complexity to $\widetilde{O}\hspace{-0.1cm}\left(\frac{nk}{\epsilon}\right)$ 

\begin{lemma}(Sample Complexity.)
\label{lem:sample_complexity}
The total number of entries of $\AA$ read by Algorithm \ref{alg:adaptive} is $\widetilde{O}\hspace{-0.1cm}\left(\frac{nk}{\epsilon}\right)$. 
\end{lemma}
\begin{proof}
Observe, $\BB^t_{i,*}$ is a $\frac{n}{2^t} \times n$ matrix. Reading $r_t$ entries in each row corresponds to querying $r_t \cdot \frac{n}{2^t} = \frac{nk \log(n)}{\epsilon}$ entries in $\AA$. Since there we repeat this for all  $t \in [\log(n)]$, the total number of entries read in $\AA$ by Step 1(a) are $\widetilde{O}\hspace{-0.1cm}\left(\frac{nk}{\epsilon}\right)$. Let the subsampled matrix be denoted by $\CC^t$. 

\noindent We then partition $\CC^t$ into level sets such that for all $\ell \in [\log(n)]$, all entries in $\DD^{t,\ell}$ have absolute value in the range  $\left( \frac{1}{2^{\ell+1}}, \frac{1}{2^{\ell+1}} \right]$. It remains to show that for any $\BB^t$, the total number of rows for which we observe a constant number of entries in $\DD^{t,\ell}$ is $\widetilde{O}\hspace{-0.1cm}\left(\frac{k}{\epsilon}\right)$. 
Assuming the above claim holds, we query $\widetilde{O}\hspace{-0.1cm}\left(\frac{nk}{\epsilon}\right)$ entries in $\AA$. It is then easy to obtain the final sample complexity bound since we simply repeat the computation for each $t, \ell  \in [\log(n)]$. 

\noindent Observe, when the rows of $\AA$ have many non-zero entries, $\DD^{t,\ell}$ can have more than a constant non-zeros in every row and thus $\S_{t,\ell}$ could be as large as $n$. For instance, the all $1$s matrix satisfies this criteria for appropriately selected $\ell$. Therefore, we introduce $\R_{t,\ell}$, a uniform subset of $\S_{t,\ell}$ with cardinality at most $\frac{k \log(n)}{\epsilon}$. This ensures Algorithm \ref{alg:adaptive} only reads $\frac{nk \log(n)}{\epsilon}$ entries in $\AA$, for a fixed  $t$ and $\ell$.  



\begin{comment}
Consider the $i$-th row of $\DD^{t,\ell}$ s.t. it corresponds to row $\AA_{i',*}$. 
The probability that the algorithm observes an entry in  $\DD^{t,\ell}_{i,*}$ is  
\begin{equation}
\label{eqn:row_expec}
    \expecf{}{X_i} = n \sum_{j\in[n]}\frac{(\BB^t_{i,j})^2}{n} = \|\BB^t_{i,j}\|^2_2 
\end{equation}
Further, $\frac{r_t}{n} X_{i,j} = (\BB^{t}_{i,j})^2 \in [0,1]$. Therefore, for all rows such that $\|\BB^t_{i,*}\|^2_2 \geq \frac{\| \AA\|^2_F}{2^{t+1}}$, by a Chernoff bound
\begin{equation*}
\begin{split}
    \Pr\left[X_i \geq (1+\eta) \|\BB^t_{i,*}\|^2_2\right] & = \Pr\left[ \frac{r_t}{n} X_i \geq (1+\eta) \frac{r_t}{n} \|\BB^t_{i,*}\|^2_2\right] \\
    &\leq \exp\left(-\frac{\eta r_t \|\BB^t_{i,*}\|^2_2 }{ 3 n} \right) \\
    & \leq \exp\left(-\frac{\eta \|\AA\|^2_F k \log(n)}{ 3\epsilon  n} \right)\\
    & \leq \frac{1}{\poly(n)}
\end{split}
\end{equation*}
where we use that $\|\AA\|^2_F \geq n$ since the diagonal is all $1$s and set $\eta$ to be a small constant. Union bounding over all such $i$, we have with probability at least $1 - \frac{1}{\poly(n)}$, $X_i = O(\log(n) \|\BB^t_{i,j}\|^2_2)$. \textcolor{red}{\textbf{Here, for all rows with small norm, we cannot obtain a strong upper bound on the corresponding estimator. So we can only control how many such rows may satisfy the threshold in expectation.}}
%Therefore, the total number of entries read in $\AA$ are $\widetilde{O}\hspace{-0.1cm}\left(\frac{nk}{\epsilon}\right)$.
\end{comment}
\end{proof}

\noindent It is well known that sampling proportional to row norms, it suffices to output a set of $\frac{k}{\epsilon}$ rows of the input matrix to recover an additive low-rank approximation \cite{fkv04, indyk2019sample}. Therefore, we show that the rows output by Algorithm \ref{alg:adaptive} match the probability distribution of the rows output by Frize-Kannan-Vempala \cite{fkv04}. To this end, we first partition  rows of $\AA$ into $\log(n)$ buckets, i.e. for all $r \in [\log(n)]$, let $$\T_{r} = \left\{ i : \frac{\|\AA\|_F}{2^{r+1}} \leq \|\AA_{i,*}\|^2_2 \leq \frac{\|\AA\|_F}{2^{r}} \right\}$$
Let the contribution of $\T_r$ to the overall Frobenius of $\AA$ be $\alpha_r$, i.e. $\alpha_r =\frac{\sum_{i\in\T_r} \|\AA_{i,*}\|^2_2 }{\|\AA \|^2_F}$. Observe, sampling $\frac{k}{\epsilon}$ rows proportional to their row norms results in sampling $\frac{\alpha_r k}{\epsilon}$ rows uniformly from $\T_r$. Formally,


 

\begin{lemma}(Effective Row Norm Sampling.)
\label{lem:effectiive_sampling}
For all $r \in [\log(n)]$, let $\T_{r} = \left\{ i : \frac{\|\AA\|_F}{2^{r+1}} \leq \|\AA_{i,*}\|^2_2 \leq \frac{\|\AA\|_F}{2^{r}} \right\}$. Let $\alpha_r = \frac{\sum_{i \in \T_{r}} \|\AA_{i,*}\|^2_2}{\|\AA\|^2_F}$ be the fractional contribution of rows in $\T_r$ to the Frobenius norm. Then, with probability at least $1 - \frac{1}{\poly(n)}$, for all $r$, Algorithm \ref{alg:adaptive} recovers at least $\frac{c_{r}k}{\epsilon}$ rows from $\T_{r}$, uniformly at random. 
\end{lemma}
\begin{proof}
First, we lower bound the cardinality of $\T_{r}$. Observe, since $\T_{r}$ contributes a $\alpha_{r}$ fraction to $\|\AA \|^2_F$ and each row has norm at least $\frac{\|\AA\|_F}{2^{r+1}}$,  $|\T_{r}| \geq \alpha_{r} 2^{r} \|\AA\|_F$. 
%Note, we only consider $\T_r$ such that $\alpha_r \geq \frac{\log(n)}{\|\AA\|_F}$ as we can discard the contribution from the remaining sets and \textcolor{red}{why is this ok?}. 
%Since the $\xi_i$'s are independent, by Chernoff,
For all $i \in \T_r$, let $\xi_i$ be the indicator random variable for row $ \AA_{i,*}$ being sampled in $\BB^t$. Then, $\Pr[\xi_i = 1] = \frac{1}{2^t}$. Let $\xi= \sum_{i \in \T_r} \xi_i$ and thus
$$\expecf{}{\xi} = \expecf{}{ \sum_{i \in \T_r} \xi_i} = \frac{|\T_r|}{2^t} \geq \frac{\alpha_r 2^{r} \| \AA \|_F}{2^t}$$
Since each of the $\xi_i$'s are independent, by Chernoff, we have 
\begin{equation}
    \begin{split}
        \Pr\left[\xi \leq (1-\eta)\expecf{}{\xi} \right] & \leq \exp\left(-\frac{\eta^2 \expecf{}{\xi}}{3} \right) \\
        & \leq \exp\left(-\frac{\eta^2 \alpha_r 2^r \|\AA\|_F}{2^t} \right) \\
        & \leq \frac{1}{\poly(n)}
    \end{split}
\end{equation}
where the last inequality follows for all $t$ such that $2^t \leq \frac{\alpha_r 2^r \|\AA \|_F}{\log(n)}$ and $\eta$ to be a small constant.  Union bounding over such events for each $r$, with probability at least $1 - \frac{1}{\poly(n)}$, $\BB^t_{i,*}$ contains at least $\frac{|\T_r|}{2^t} \geq \frac{\alpha_r 2^{r} \| \AA \|_F}{2^t}$ rows from $\T_r$. Let the restriction of the matrix $\BB^t$ to the set of rows in $\T_r$ be denoted by $\BB^t_{\T_r}$. 

Consider the case when $t=r$. Let $\b_{i,*}$ denote the  $i$-th row in $\BB^t_{\T_r}$. Then, for all $i \in \left[\frac{n}{2^t}\right]$, there exists $\ell$ such that at least a $\frac{1}{\log(n)}$ fraction of the $\ell^2_2$ norm of $\b_{i,*}$ has absolute values in the range $\left( \frac{1}{2^{\ell+1}}, \frac{1}{2^\ell}\right]$. The minimum number of entries in this row with absolute value at most $\frac{1}{2^{\ell}}$ is at least $\frac{\|\AA\|_F 2^{\ell}}{2^{r+1}\log(n)}$. Recall, we construct $\CC^{t}$ by uniformly sampling entries in $\BB^t$. We would like to lower bound the number of entries in $\CC^t_{i,*}$ such that the corresponding entry in $\b_{i,*}$ has absolute value in the range $\left( \frac{1}{2^{\ell+1}}, \frac{1}{2^\ell}\right]$. Observe, $$\Pr\left[ \CC^t_{i,j}  = \b_{i,j'} \textrm{ } \Big{|} \textrm{ } \b_{i,j'}^2 \in  \left( \frac{1}{2^{\ell+1}}, \frac{1}{2^\ell}\right]\right] \geq  \frac{\|\AA\|_F 2^{\ell}}{2^{r+1}n\log(n)} $$ 
We repeat the above sampling $\frac{2^t k \log^2(n)}{\epsilon}$ times, and denote the resulting set by $\DD^{t,\ell}_{i,*}$. Then,
\begin{equation}
\label{eqn:card_lb}
    \begin{split}
        \Pr\left[|\DD^{t,\ell}_{i,*}| \geq 1 \right] &= 1- \Pr\left[|\DD^{t,\ell}_{i,*}| = 0 \right] \\
        & = 1 - \left(1- \Pr\left[ \CC^t_{i,1}  = \b_{i,j'} \textrm{ } \Big{|} \textrm{ } \b_{i,j'}^2 \in  \left( \frac{1}{2^{\ell+1}}, \frac{1}{2^\ell}\right]\right]\right)^{\frac{2^tk\log^2(n)}{\epsilon}}\\
        %\expecf{}{|\DD^{t,\ell}_{i,*}|} & = \sum_{j \in \left[\frac{2^tk\log(n)}{\epsilon}\right]} \Pr\left[ \CC^t_{i,j}  = \b_{i,j'} \textrm{ } \Big{|} \textrm{ } \b_{i,j'}^2 \in  \left( \frac{1}{2^{\ell+1}}, \frac{1}{2^\ell}\right]\right] \\ 
        & \geq \left( \frac{\|\AA\|_F 2^{\ell}}{2^{r+1}n\log(n)}\right) \cdot \left(\frac{2^tk\log^2(n)}{\epsilon} \right) 
    \end{split}
\end{equation}
Here, we used Bernoulli's inequality.  
\begin{comment}
Since each entry of $\DD^{t,\ell}$ is sampled independently, by Chernoff, we have 
\begin{equation}
    \begin{split}
    \Pr\left[ |\DD^{t,\ell}| \leq (1-\eta)\expecf{}{|\DD^{t,\ell}|}  \right] & \leq \exp\left(-\frac{\eta^2\expecf{}{|\DD^{t,\ell}|} }{3}\right) \\
    & \leq \exp\left(- \frac{\eta^2 \|\AA\|_F 2^{\ell} 2^t k \log(n)}{2^{r+1}\epsilon n} \right)
    \end{split}
\end{equation}
Setting $\eta$ to be a small constant $<1$, we can union bound over all such events for  $n$ rows of $\AA$ such that with probability $1-\frac{1}{\poly(n)}$, simultaneously for all rows of $\AA$, there exists $\DD^{t,\ell}$ such that
\begin{equation}
\label{eqn:card_lb}
    \begin{split}
    \Pr\left[ |\DD^{t,\ell}| \geq \frac{1}{2}\expecf{}{|\DD^{t,\ell}|}  \right] & \geq 1 - \exp\left(- \frac{ \|\AA\|_F 2^{\ell} 2^t k }{2^{r+1}\epsilon n} \right) \\
    & \geq \frac{ \|\AA\|_F 2^{\ell} 2^t k }{2^{r+1}\epsilon n}
    \end{split}
\end{equation}
\end{comment}
Unfortunately, the above probability could be as small as $1/n$, obtaining a trivial bound when $\|\AA \|_F$ is small. Here, it is useful to consider the instance where $\AA$ has a diagonal of all $1$s and $\sqrt{n}$ rows with $\sqrt{n}$ $1$s on the off-diagonal. Here, the $\sqrt{n} \times \sqrt{n}$ block contributes a constant fraction of the overall Frobenius norm and we cannot ignore it. For any row in this block, $\frac{\| \AA\|_F}{2^{r+1}} = \sqrt{n}$ and $2^\ell \leq O(1)$. Setting $t$ such that $2^t = \sqrt{n}$, only $O(1)$ rows from the block remain as opposed to $\Theta\left(\frac{k}{\epsilon}\right)$  rows that \cite{fkv04} recovers. 

\noindent While we cannot obtain tight concentration for a row wise guarantee, we can show that at least $\alpha_r \frac{k}{\epsilon} $ rows from $\T_r$ correspond to a $\DD^{t,\ell}_{i,*}$ that has cardinality at least $1$, with constant cardinality. This suffices to detect the right number of rows from $\T_r$ to match \cite{fkv04}. Let $\zeta_i$ be an indicator random variable for the event that for row $b_i$, there exists an appropriate level set $\DD^{t,\ell}_{i,*}$ such that $|\DD^{t,\ell}| \geq 1$. Then, from Equation \ref{eqn:card_lb} $\Pr[\zeta_i=1] \geq \frac{ \|\AA\|_F 2^{\ell} 2^t k \log^2(n) }{2^{r+1}\epsilon n}$. Since $\BB^t$ contains at least $\frac{|\T_r|}{2^t}$ rows,  
\begin{equation*}
    \expecf{}{\sum_{i \in \left[\frac{|\T_r|}{2^t}\right]}\zeta_i} \geq \left( \frac{ \|\AA\|_F 2^{\ell} 2^t k \log^2(n) }{2^{r+1}\epsilon n}\right) \cdot \left(  \frac{\alpha_r 2^{r} \| \AA \|_F}{2^t}\right) \geq \frac{ \alpha_r \|\AA\|^2_F 2^{\ell}  k \log^2(n)}{4 \epsilon n } \geq \frac{ \alpha_r k \log^2(n)}{4 \epsilon  }
\end{equation*}
%\textcolor{red}{propogate the $log^2$ back up in sample complexity.}
where the last inequality follows from $\|\AA \|^2_F \geq n$ and $\frac{1}{2^\ell} \leq 1$. While we do not obtain exponential concentration, by Markov's inequality, with probability $ 1 - \frac{1}{100\log^2(n)}$, 
$$ \sum_{i \in \left[\frac{|\T_r|}{2^t}\right]}\zeta_i \geq \frac{1}{100\log^2(n)} \expecf{}{\sum_{i \in \left[\frac{|\T_r|}{2^t}\right]}\zeta_i} \geq \frac{\alpha_r k}{\epsilon} $$
Observe, for at least $\frac{\alpha_rk}{\epsilon}$ rows, there exists $t, \ell$ such that the corresponding row in $\DD^{t,\ell}$ has cardinality at least $1$. 
%thus been able to detect the right number of rows in $\T_r$. 
We then union bound over all $\log^2(n)$ values of $t$ and $\ell$ such that with probability at least $\frac{99}{100}$, Algorithm \ref{alg:adaptive} detects at least $ \frac{\alpha_r k }{\epsilon}$ rows from $\T_r$.  \textcolor{red}{remains to show we obtain these rows uniformly from $T_r$.}

\textcolor{red}{Now that we have showed for the right setting of $\ell$ and $t$ we recover at least $\frac{\alpha_r k}{\epsilon}$ rows from $\T_r$, it remains to show that for any other setting of $t$ and $\ell$, we recover at most $\alpha_r \frac{k}{\epsilon}$ rows from $\T_r$. }
Since each row in $\T_r$ has norm at least $\frac{\|\AA \|_F}{2^{r+1}}$, we have $|\T_r| \leq \alpha_r 2^{r+1}\|\AA \|_F$. As before, for all $i \in \T_r$, let $\xi_i$ be the indicator random variable for row $ \AA_{i,*}$ being sampled in $\BB^t$. Then, $\Pr[\xi_i = 1] = \frac{1}{2^t}$. Let $\xi= \sum_{i \in \T_r} \xi_i$ and thus
$$\expecf{}{\xi} = \expecf{}{ \sum_{i \in \T_r} \xi_i} = \frac{|\T_r|}{2^t} \leq \frac{\alpha_r 2^{r+1} \| \AA \|_F}{2^t}$$
Following equation \ref{}  we have 
\begin{equation}
    \begin{split}
        \Pr\left[\xi \geq (1+\eta)\expecf{}{\xi} \right] & \leq \frac{1}{\poly(n)}
    \end{split}
\end{equation}
Then, setting $\eta$ to be a small constant,  with probability at least $1 - \frac{1}{\poly(n)}$, for all $r \in [\log(n)]$, $\BB^{t}$ contains at most $O\left(\frac{\alpha_r 2^{r+1} \|\AA \|_F}{2^t}\right)$ rows from $\T_r$. For each such row, $\b_i$, the number of entries with absolute value in the range $\left(\frac{1}{2^{\ell+1}}, \frac{1}{2^{\ell}} \right]$ is at most $O\left(\frac{ 2^{\ell+1} \| \AA \|_F }{2^{r}}\right)$. The probability that the algorithm observes at least $1$ entry in $\b_i$ is then 
\begin{equation}
\begin{split}
    \Pr\left[ |\DD^{t, \ell}_{i,*}| \geq 1 \right] & \leq 1 - \left(1-\frac{ 2^{\ell+1} \| \AA \|_F }{2^{r}n}\right)^{\frac{2^t k}{\epsilon}}  \\
    & \leq \frac{ 2^t k 2^{\ell+1} \| \AA \|_F }{2^{r} \epsilon n}
\end{split}
\end{equation}
As before, let $\zeta_i$ be an indicator random variable for the event that for row $b_i$, for any level set $\DD^{t,\ell}_{i,*}$, from Equation \ref{eqn:card_lb} we have  $$\Pr[\zeta_i=1] \leq \frac{ 2^t k 2^{\ell+1} \| \AA \|_F }{2^{r} \epsilon n}$$ 
Let $\zeta = \sum_{i \in \T_r} \zeta_i$. Since, with probability at least $1-\frac{1}{\poly(n)}$, $\BB^t$ contains at most $\frac{\alpha_r 2^{r+1}\|\AA\|_F}{2^t}$ rows from $\T_r$,  
\begin{equation}
    \expecf{}{\zeta} = \expecf{}{\sum_{i\in \T_r} \zeta_i} \leq \frac{ 2^t k 2^{\ell+1} \| \AA \|_F }{2^{r} \epsilon n} \cdot \frac{\alpha_r 2^{r+1}\|\AA\|_F}{2^t} \leq \frac{\alpha_r 2^{l} \| \AA\|^2_F k}{\epsilon n}
\end{equation}
Then, by Markov's inequality,
$$\Pr\left[ \zeta \geq c\log^2(n) \expecf{}{\zeta}  \right] \leq \frac{1}{\log^2(n)}$$
Then, union bounding over all such events for $\log^2(n)$ values of $\ell$ and $t$, with probability at least $99/100$, for all $t,r$, for any $\ell$, Algorithm \ref{alg:adaptive} observes more than one non-zero entry for  at most $\widetilde{O}\left(\frac{\alpha_r 2^{l} \| \AA\|^2_F k}{\epsilon n}\right)$ rows from $\T_r$. 

\noindent It now remains to show that there exists $t,\ell$ such that $\R_{t,\ell}$ contains at least $\frac{\alpha_r k}{\epsilon}$ rows selected uniformly from $\T_r$ and $|\R_{t,\ell}| \leq \widetilde{O} \left( \frac{k}{\epsilon}\right)$. It then follows that we read $\widetilde{O} \left( \frac{nk}{\epsilon}\right)$ entries in $\AA$ to certify $\Omega\left(\frac{\alpha_r k}{\epsilon}\right)$ from $\T_r$ and add them to the set $\I_t$, which would conclude the proof. As shown above, with probability $99/100$, there exists $t, \ell^*$ s.t. $\S_{t,\ell^*}$ contains at least $\frac{\alpha_r 2^l \|\AA \|^2_F}{\epsilon n}$ rows from $\T_r$ and for all $r' \neq r$, $\S_{t,\ell^*}$ contains at most $\widetilde{O}\left(\frac{\alpha_{r'} 2^{l} \| \AA\|^2_F}{n}\right)$ from $\T_{r'}$. However, the first challenge here is that $\alpha_r$ and $\alpha_{r'}$ can differ by a polynomial factor in $n$. Therefore, it might be the case that picking $\frac{k}{\epsilon}$ rows in $\S_{t,\ell}$ uniformly at random results in no rows from $\T_r$ being selected. \textcolor{red}{The second challenge is to show that each row in $\T_r$ has equal probability of being sampled in $\R_{t,\ell}$.}


\noindent We first note that we can ignore all $\T_r$ such that $\alpha_r \leq \frac{1}{\poly{\log(n)}}$. Then, we can over sample by a $\poly{\log(n)}$ factor to ensure the right number of rows exist in $\R_{t,\ell}$. Formally, 

%contains $\Theta(c_{r} \|\AA\|_F)$ rows from $\T_{r}$. Next, we show that with probability at least $1- \frac{1}{\poly(n)}$, we estimate the row norms of at least $\frac{c_r k}{\epsilon}$ rows up to a small constant. Recall, by equation \ref{eqn:row_expec}, $\expecf{}{X_i} = \|\BB^{t}_{i,*}\|^2_2$. Let $i'$ be the row in $\AA$ corresponding to row $\BB^{t}_{i,*}$. Observe, $\var{X_i} = r_t \var{X_{i,j}} \leq r_t \expecf{}{X^2_{i,j}}$. Then, 
\begin{comment}
\begin{equation}
    \var{X_i} \leq r_t \sum_{j \in [n]} \frac{n}{r_t^2} (\BB^t_{i,j})^4 \leq \frac{n}{r_t} \sum_{j \in [n]} (\BB^t_{i,j})^2 \AA_{i',i'} \AA_{j,j} = \frac{n}{r_t} \|\BB^t_{i,*} \|^2_2
\end{equation}
where the last inequality follows from recalling that $\BB^{t}_i$ corresponding to some row $i'$ in $\AA$ and thus by Cauchy-Schwarz, $\AA^4_{i',j} \leq \AA^2_{i',j} \AA_{i',i'} \AA_{j,j}$. Similarly, $|X_{i,j}| \leq \frac{n}{r_t} \AA^2_{i',j} \leq \frac{n}{r_t} \AA_{i',i'}\AA_{j,j}$. Using Bernstein's inequality, we have 
\begin{equation}
\begin{split}
    \Pr \left[ X_i \geq (1+\eta)\|\BB^{t}_{i,*}\|^2_2 \right] & \leq \exp \left( - \frac{\eta^2 \|\BB^{t}_{i,*}\|^4_2 }{\frac{n}{r_t} \|\BB^t_{i,*} \|^2_2 + \frac{\eta\|\BB^{t}_{i,*}\|^2_2 n}{r_t}  }\right)\\
    & \leq \exp \left( - \frac{\eta^2 \|\BB^{t}_{i,*}\|^2_2 r_t }{ 2n }\right)\\
    & \leq \exp \left( - \frac{\eta^2 \|\AA \|_F k \log^2(n) }{ 2 \epsilon n }\right) \\
    & \leq \frac{1}{\poly(n)}\exp \left( - \frac{ \|\AA \|_F k \log(n) }{ 2 \epsilon n }\right) 
\end{split}
\end{equation}
Then, setting $\eta$ to be a small constant and union bounding over all rows in $\T_{r}$, we have for all $i \in \T_r$, $X_i = \Theta(\|\BB^{t}_{i,*}\|^2_2)$ with probability at least $1 - \exp \left( - \frac{ \|\AA \|_F k \log(n) }{  \epsilon n }\right) \geq \frac{ \|\AA \|_F k \log(n) }{  \epsilon n }$. \textcolor{red}{Insert Chernoff here.} Since, $\BB^t$ contains at least  $ c_{r} \|\AA\|_F$ rows from $\T_r$, with probability $1- \frac{1}{\poly(n)}$, for at least $\frac{ \|\AA \|_F k \log(n) }{  \epsilon n } \cdot c_{r} \|\AA\|_F \geq \frac{c_t k\log(n)}{\epsilon}$ rows, $X_i = \Theta(\|\BB^{t}_{i,*}\|^2_2)$. In the last inequality, we used that $\|\AA \|^2_F \geq n$. 


\noindent Therefore, at least $\frac{c_t k\log(n)}{\epsilon}$ rows from $\T_r$ satisfy the threshold and upon reading all of them we can certify that they indeed belong to $\T_r$. We then conclude that Algorithm \ref{alg:adaptive} indeed samples the right number of rows from each level set, and thus matches the output distribution of row-norm sampling. 
\end{comment}
\end{proof}

\noindent From Lemma \ref{lem:sample_complexity} and Lemma \ref{lem:effectiive_sampling}, it follows that Algorithm \ref{alg:adaptive} matches the distributions over rows of Frieze-Kannan-Vempala \cite{fkv04}. Therefore, following the argument Frieze-Kannan-Vempala the span of the $\widetilde{O}\hspace{-0.1cm}\left(\frac{k}{\epsilon}\right)$, rows sampled by Algorithm \ref{alg:adaptive} contains a good additive-error low-rank approximation to $\AA$.  



==> bicriteria.tex <==
\newpage
\section{Relative Error Bi-criteria LRA}

\begin{lemma}
Let $\MM$ be a rank-$r$ matrix and let $\MM_i$ be the $i$-th row of $\MM$. Let $\tau_i(\MM) = \MM_{i}^T (\MM \MM^T)^{+} \MM_i$ be the $i$-th leverage score of $\MM$. Then, $\sum_i \tau_{i}(\MM) = r$. 
\end{lemma}


\begin{lemma}(Mixture PCP.)
Let $\AA$ be a $n \times n$ PSD matrix and $\BB = \UU \UU^T$ be an $O(1)$-approximate low-rank approximation to $\AA$, i.e. $\|\AA - \UU \UU^T\|^2_F \leq O(1)\|\AA -\AA_k \|^2_F$. Let $q = \{q_1, q_2 \ldots q_n\}$ be a probability distribution over the columns of $\AA - \BB$, such that for all $j$, $q_j =  \frac{1}{2n}+\frac{\tau_{j}(\BB)}{2 \sum_j \tau_j(\BB)}$, where $\tau_j(\BB)$ is the $j$-th leverage score of $\BB$.  Let $t =  O\left(\sqrt{nk}\log(n/\delta)/\epsilon^2\right)$. Then, construct $\CC$ using $t$ columns of $\AA-\BB$ and set each one to $(\AA-\BB)_{*,j}/\sqrt{t q_j}$ with probability $q_j$. With probability at least $1-\delta$, for any rank-$k$ orthogonal projection $\XX$,
\[
(1-\epsilon)(\AA-\BB)(\AA-\BB)^T  - \frac{\epsilon}{k}\| \AA\|^2_F \II \preceq \CC \CC^T \preceq (1+\epsilon)(\AA-\BB)(\AA-\BB)^T +  \frac{\epsilon}{k}\| \AA\|^2_F\II
\]
\end{lemma}
\begin{proof}
Let $\Y = \CC\CC^T - (\AA-\BB)(\AA-\BB)^T$. For notational convenience let $(\AA-\BB)_j = (\AA-\BB)_{*,j}$. We can then write $\Y = \sum_{j \in [t]} \left(\CC_{*,j} \CC_{*,j}^T -\frac{1}{t}(\AA-\BB)(\AA-\BB)^T\right) = \sum_{j\in [t]} \XX_j$, where $\XX_j = \frac{1}{t}(\frac{1}{q_j}(\AA-\BB)_{j}(\AA-\BB)^T_{j} - (\AA-\BB)(\AA-\BB)^T )$ with probability $q_j$. We observe that $\expec{}{\XX_j} = \expec{}{\CC_{*,j} \CC_{*,j}^T -\frac{1}{t}(\AA-\BB)(\AA-\BB)^T}=  0$, and therefore, $\expec{}{\Y} =0$. Next, we bound the operator norm of $\Y$. To this end, we use the Matrix Bernstein inequality, which in turn requires a bound on the operator norm of $\XX_j$ and variance of $\Y$. 
Recall, 
\begin{equation}
\label{eqn:spec_x_j}
    \begin{split}
        \| \XX_j \|_2 & = \left\| \frac{1}{tq_j}(\AA-\BB)_{j}(\AA-\BB)_{j} - \frac{1}{t}(\AA-\BB)(\AA-\BB)^T \right\|_2 \\
        &\leq  \frac{1}{t}\left(\frac{1}{2n} + \frac{\tau_i(\BB)}{2k} \right)^{-1} \|(\AA-\BB)_{j}\|^2_2 + \frac{1}{t} \| \AA-\BB\|^2_2\\
        %& \leq \frac{2n}{t(1+\tau_j(\BB))}\left(\|\AA_j\|^2_2+\| \BB_{j} \|^2_2 \right) + \frac{1}{t}\| \AA\|^2_2 \\
        %& \leq \frac{2n}{t(1+\tau_j(\BB))}\left(\|\AA\|_2+\| \BB_{j} \|^2_2 \right)  + \frac{n}{t}\| \AA\|_2  \\
        %&  \leq \frac{3n}{t(1+\tau_j(\BB))}\left(\|\AA\|_2+\| \BB_{j} \|^2_2 \right) \\
    \end{split}
\end{equation}
where we use triangle inequality for operator norm, $\|\AA_j \|^2_2\leq \| \AA \|_2$, $\|\AA\|_F \leq n$ and that $\| \AA +\NN \|_2 \leq \trace{\AA+ \NN}\leq n + \epsilon\|\AA\|^2_F$. 
Next, we bound $\var{\Y}\leq \expecf{}{\Y^2}$.

\begin{equation}
    \begin{split}
        \expecf{}{\Y^2}  & =  t\expecf{}{\left(\CC_{*,j} \CC_{*,j}^T -\frac{1}{t}(\AA-\BB)(\AA-\BB)^T\right)^2} \\
        & = t\expecf{}{ \left(\CC_{*,j} \CC_{*,j}^T\right)^2 +\frac{1}{t^2}\left((\AA-\BB)(\AA-\BB)^T\right)^2 - \frac{2}{t}\CC_{*,j} \CC_{*,j}^T (\AA-\BB)(\AA-\BB)^T } \\
        %& = \left(\sum_{j \in [n]} \frac{1}{tq_j} ((\AA-\BB)_{j}(\AA-\BB)^T_{j})^2 + \frac{1}{t}((\AA-\BB)(\AA-\BB)^T)^2 - \sum_{j \in [n]} \frac{1}{t}(\AA-\BB)_j (\AA-\BB)_j^T (\AA-\BB)(\AA-\BB)^T \right) \\
        %& = \frac{1}{t}\left( \sum_{j \in [n]} \frac{((\AA-\BB)_{j}(\AA-\BB)^T_{j})^2}{q_j} + ((\AA-\BB)(\AA-\BB)^T)^2 - \sum_{j \in [n]} 2 (\AA-\BB)_{j}(\AA-\BB)^T_{j} (\AA-\BB)(\AA-\BB)^T \right) \\
        & = \frac{1}{t}\left( \sum_{j \in [n]} \frac{((\AA-\BB)_{j}(\AA-\BB)^T_{j})^2}{q_j} - ((\AA-\BB)(\AA-\BB)^T)^2 \right) \\
        & \preceq \frac{n}{t(1+\tau_j(\BB))}\left( \sum_{j \in [n]}  ((\AA-\BB)_{j}(\AA-\BB)^T_{j})^2 \right) \\
        & \preceq \frac{n}{t(1+\tau_j(\BB))}\left( \sum_{j \in [n]} \left(\|\AA \|_2 + \|\BB_j\|^2_2\right) (\AA-\BB)_{j}(\AA-\BB)^T_{j} \right) \\
        & \preceq \frac{cn\left(\|\AA \|_2 + \|\BB_j\|^2_2\right)}{t(1+\tau_j(\BB))} (\AA-\BB) (\AA-\BB)^T \\
        \expecf{}{\YY^2}&  \preceq \frac{cn\left(\|\AA \|_2 + \|\BB_j\|^2_2\right)}{t(1+\tau_j(\BB))} \AA \AA^T \\ 
    \end{split}
\end{equation}
where we use linearity of expectation, $(\AA\AA^T)^2 \succeq 0$ and $\|\AA_{j,*}\|^2_2\leq \| \AA\|_2\cdot \AA_{j,j}$.
Therefore, $ \| \expecf{}{\Y^2} \|_2 \leq \frac{c\trace{\AA}\| \AA\|^3_2 }{t}$. Applying the Matrix Bernstein inequality, 

\begin{equation*}
    \begin{split}
        \prob{}{\| \Y \|_2 \geq \Big\|\epsilon \AA\AA^T  +  \frac{\epsilon}{k}\| \AA \|^2_F\II \Big\|_2 } & \leq 2n \exp{\left(- \frac{\big\|\epsilon \AA\AA^T  +  \frac{\epsilon\| \AA \|^2_F}{k}\II \big\|^2_2}{  \frac{c\trace{\AA} \|\AA \|^3_2 }{t}  +  \frac{2\trace{\AA} \|\AA\|_2 \left(\big\|\epsilon \AA\AA^T  +  \frac{\epsilon}{k}\| \AA \|^2_F\II \big\|_2 \right)}{3t} }\right)} \\
        & = 2n \exp{\left(-\frac{\epsilon^2 }{k^2 }\left(  \frac{\big\|k \AA\AA^T  + \|\AA\|^2_F \II \big\|^2_2 }{ \frac{c\trace{\AA} \|\AA \|^3_2 }{t}  +  \frac{2\epsilon \trace{\AA} \|\AA\|_2 \left(\|k \AA\AA^T  + \|\AA\|^2_F \II \|_2 \right)}{3kt}}\right) \right)} \\
        & = 2n \exp{\left(-\frac{\epsilon^2t }{c'k^2\trace{\AA} \|\AA \|_2 }\left(  \frac{\big\|k \AA\AA^T  + \|\AA\|^2_F \II \big\|^2_2 }{ \frac{ k\|\AA\AA^T \|_2 + \epsilon \|k \AA\AA^T  + \|\AA\|^2_F \II \|_2  }{k}}\right) \right)} \\
        & \leq 2n \exp{\left(-\frac{\epsilon^2t }{c'k\trace{\AA} \|\AA \|_2 }\left(  \frac{\big\|k \AA\AA^T  + \|\AA\|^2_F \II \big\|^2_2 }{(1+\epsilon) \|k \AA\AA^T  + \|\AA\|^2_F \II \|_2  }\right) \right)} \\
        %& = 2n \exp{\left(- \frac{3 \epsilon^2 \| \AA \|^2_F t}{cn \|\AA\|_2 (1+\epsilon)} \right)} \\
        & \leq 2n \exp{\left(- \frac{ \epsilon^2 t \left( \big\|k \AA\AA^T  + \|\AA\|^2_F \II \big\|_2 \right) }{c'nk \|\AA\|_2 } \right)} \\
        & \leq 2n \exp{\left(- \frac{ \epsilon^2 \sqrt{k}t \| \AA \|_2 \|\AA\|_F }{c'\trace{\AA}k \|\AA\|_2 } \right)} \hspace{0.5in} \textrm{ [A.M - G.M inequality]}\\
        %& \leq 2n \exp{\left(- \frac{3 \epsilon^2 t \sqrt{n}}{cn } \right)} \\
        & \leq 2n \exp{\left(- \frac{\epsilon^2 t}{c'\sqrt{nk} } \right)} \\
        %& \leq 2n \exp{\left(- \frac{\epsilon^2 \| \AA \|_F t}{cn} \right)} \\
        %& \leq 2n \exp{\left(- \frac{\epsilon^2  t}{c\sqrt{n}} \right)} \\
        %&\leq \delta
    \end{split}
\end{equation*}
Here, we use $\|k \AA\AA^T  + \|\AA\|^2_F \II \|_2 = k\|\AA \|^2_2 + \|\AA\|^2_F \geq 2 \sqrt{k} \|\AA \|_2\|\AA\|_F$, by the AM-GM inequality. Next, we use  $\trace{\AA}\leq \sqrt{n}\|\AA\|_F$. Recall, 
\begin{equation*}
    \begin{split}
        \trace{\AA} = \sum^n_{i=1}\sigma_i(\AA) \leq \sqrt{\sum^n_{i=1} \sigma_i^2(\AA) \cdot n} = \sqrt{ n \|\AA\|^2_F }
    \end{split}
\end{equation*}
using the Cauchy-Schwarz inequality. In order to bound the error by $\delta$ we set $t = \frac{c'\sqrt{nk}}{\epsilon^2}\log\left(\frac{2n}{\delta}\right)$. Therefore, with probability $1-\delta$, 
\[
(1-\epsilon)\AA\AA^T  - \frac{\epsilon}{k}\| \AA\|^2_F \II \preceq \CC \CC^T \preceq (1+\epsilon)\AA\AA^T +  \frac{\epsilon}{k}\| \AA\|^2_F\II
\]
\end{proof}
